Stay Positive: Non-Negative Image Synthesis for Augmented Reality

In applications such as optical see-through and projector augmented reality, producing images amounts to solving non-negative image generation, where one can only add light to an existing image. Most image generation methods, however, are ill-suited to this problem setting, as they make the assumption that one can assign arbitrary color to each pixel. In fact, naive application of existing methods fails even in simple domains such as MNIST digits, since one cannot create darker pixels by adding light. We know, however, that the human visual system can be fooled by optical illusions involving certain spatial configurations of brightness and contrast. Our key insight is that one can leverage this behavior to produce high quality images with negligible artifacts. For example, we can create the illusion of darker patches by brightening surrounding pixels. We propose a novel optimization procedure to produce images that satisfy both semantic and non-negativity constraints. Our approach can incorporate existing state-of-the-art methods, and exhibits strong performance in a variety of tasks including image-to-image translation and style transfer.

==> figures/alpha.tex <==
{\renewcommand{\tabcolsep}{1pt}
\begin{figure}
\centering
\begin{tabular}{cccc}
$\alpha=0.2$ & $\alpha=0.4$ & $\alpha=0.6$ & $\alpha=0.8$ \\
\includegraphics[width=0.24\linewidth]{figures/baseline_alpha/alpha02.png}&
\includegraphics[width=0.24\linewidth]{figures/baseline_alpha/alpha04.png}&
\includegraphics[width=0.24\linewidth]{figures/baseline_alpha/alpha06.png}&
\includegraphics[width=0.24\linewidth]{figures/baseline_alpha/alpha08.png}\\
\end{tabular}
    \caption{The effect of $\alpha$ values on the image quality.}
    \label{fig:alpha} % I can do without the label too
\end{figure}}

==> figures/tasks_compare.tex <==
{
\renewcommand{\tabcolsep}{2pt}
\begin{figure*}
\centering
\begin{tabular}{cccccc}
Day $\to$ Night~\cite{Anokhin_2020_CVPR} & 
Dog $\to$ Cat~\cite{Huang_2018_ECCV} & 
Photo $\to$ Style~\cite{huang2017adain} & 
Style $\to$ Photo~\cite{huang2017adain} & 
Sketch $\to$ Photo~\cite{huang2017adain} & 
Face $\to$ Smile~\cite{shen2020interpreting} \\
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/day2aurora/day2aurora-input.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/dog2cat/dog2cat-input.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/photo2style_avril/photo2style_avril-input.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/style2photo_chicago/style2photo_chicago-input.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/sketch2photo_sailboat/sketch2photo_sailboat-input.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/face2smile/face2smile-input.jpg} \\

\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/day2aurora/day2aurora-target.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/dog2cat/dog2cat-target.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/photo2style_avril/photo2style_avril-target.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/style2photo_chicago/style2photo_chicago-target.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/sketch2photo_sailboat/sketch2photo_sailboat-target.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/face2smile/face2smile-target.jpg} \\

\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/day2aurora/day2aurora-baseline.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/dog2cat/dog2cat-baseline.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/photo2style_avril/photo2style_avril-baseline.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/style2photo_chicago/style2photo_chicago-baseline.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/sketch2photo_sailboat/sketch2photo_sailboat-baseline.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/face2smile/face2smile-baseline.jpg} \\

\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/day2aurora/day2aurora-ours.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/dog2cat/dog2cat-ours.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/photo2style_avril/photo2style_avril-ours.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/style2photo_chicago/style2photo_chicago-ours.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/sketch2photo_sailboat/sketch2photo_sailboat-ours.jpg}&
\includegraphics[width=0.16\textwidth]{figures/tasks_comparison/face2smile/face2smile-ours.jpg} \\

\end{tabular}
\caption{We compare our results across a variety of domains. From top to bottom: input, proposal, heuristic baseline, our method.}
\label{fig:resid} % I can do without the label too
\end{figure*}
}

==> tables/deprecated/ablation_norms.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|lll}
 & FID & PSNR (?) & Broken Pixels \\ \hline \hline
Basic norm & 139.1359 & 20.4047 & 0.2273 \\
Moment norm & 143.9986 & 20.0339 & 0.1549 \\
No normalization & 146.9467 & 26.5927 & 0.5001 \\
KDE norm &  &  & 
\end{tabular}
\caption{Claim 7: ablation study on normalizaiton methods}
\label{tab:ablation-norms}
\end{table}

==> tables/deprecated/ablations_param.tex <==
\begin{table}[]
\centering
\begin{tabular}{l|lll}
 & FID & PSNR & Broken Pixels \\ \hline \hline
Pixel Offset & 132.8215 & 19.7896 & 0.2305 \\
Group Offset & 125.7491 & 20.5588 & 0.2133 \\
Channel Offset & 139.1359 & 20.4047 & 0.2273 \\
Single Offset & 126.2443 & 20.6763 & 0.2114
\end{tabular}
\caption{Claim 3: ablation study on  different ways to offsets }
\label{tab:ablations-params}
\end{table}

==> tables/deprecated/image_translation.tex <==
\begin{table}
\centering
\begin{tabular}{l c c c c} 
 & PNSR & FID & Norm. L1 & \% OOD Pix. \\ 
 \hline\hline
 GAN (no norm) & \\
 GAN (norm) & \\
 \hline
 Heuristic & \\
 Ours (no norm) & \\
 \hline
 \textbf{Ours}
\end{tabular}
\caption{Table template 1}
\label{table:1}
\end{table}

==> tables/deprecated/sat2map.tex <==
\begin{table}
\centering
\begin{tabular}{l | c c c | c c c} 
 & \multicolumn{3}{c |}{Map $\rightarrow$ Satellite} & \multicolumn{3}{c}{Satellite $\rightarrow$ Map}\\
 & FID & PNSR & \% OOD Pix. & FID & PNSR & \% OOD Pix. \\ 
 \hline
 Heuristic & \\
 \textbf{Ours}
\end{tabular}
\caption{Table template 2}
\label{table:3}
\end{table}

==> tables/deprecated/task_styletransfer.tex <==
% \begin{table}
% \centering
% \begin{tabular}{l | c c | c c} 
%  & \multicolumn{2}{c |}{Monet $\rightarrow$ Photo} & \multicolumn{2}{c}{Photo $\rightarrow$ Monet}\\
%  & PNSR & \% OOD Pix. & PNSR & \% OOD Pix. \\ 
%  \hline
%  Heuristic & \\
%  \textbf{Ours}
% \end{tabular}
% \caption{Table template 2}
% \label{table:2}
% \end{table}
\begin{table}
\centering
\begin{tabular}{l|lll}
 & VonGogh & Cezanne & Uyeoko \\ \hline \hline
Heuristic & 124.5744 & 223.2128 & 206.7694 \\
Ours & 120.1159 & 219.0010 & 196.1496
\end{tabular}
\caption{Claims 2: our model can work with a wide range of tasks}
\label{tab:styletransfer}
\end{table}
